NeuralODF: Learning Omnidirectional Distance Fields for 3D Shape Representation

In visual computing, 3D geometry is represented in many different forms including meshes, point clouds, voxel grids, level sets, and depth images. Each representation is suited for different tasks thus making the transformation of one representation into another (forward map) an important and common problem. We propose Omnidirectional Distance Fields (ODFs), a new 3D shape representation that encodes geometry by storing the depth to the object's surface from any 3D position in any viewing direction. Since rays are the fundamental unit of an ODF, it can be used to easily transform to and from common 3D representations like meshes or point clouds. Different from level set methods that are limited to representing closed surfaces, ODFs are unsigned and can thus model open surfaces (e.g., garments). We demonstrate that ODFs can be effectively learned with a neural network (NeuralODF) despite the inherent discontinuities at occlusion boundaries. We also introduce efficient forward mapping algorithms for transforming ODFs to and from common 3D representations. Specifically, we introduce an efficient Jumping Cubes algorithm for generating meshes from ODFs. Experiments demonstrate that NeuralODF can learn to capture high-quality shape by overfitting to a single object, and also learn to generalize on common shape categories.

==> tables/ablation1.tex <==
\setlength{\tabcolsep}{4pt}
\begin{table}
%\centering
\begin{minipage}[b]{0.45\linewidth}\centering
    
    \scalebox{0.8}{
    \begin{tabular}{c|c|cc}
    %\hline
    \specialrule{.1em}{.1em}{.1em}
    Iter. & \multicolumn{1}{c}{Depth Metrics} & \multicolumn{2}{|c}{Intersection Conf. Metrics} \\
    & CD $\downarrow$  & Rec. $\uparrow$ (\%) & F-score (\%) $\uparrow$  \\ %\hline
    \specialrule{.1em}{.1em}{.1em}
     1  & 0.425  & 59.41  & 72.66\\
     3  & 0.302  & 96.29 & 94.65\\
     5  & 0.351  & 96.40 & 94.62\\
     %7  & 0.362  & 96.37 & 94.60\\
     %9  & 0.364  & 96.56 & 94.70\\
     %11 & 0.368  & \textbf{96.83} & \textbf{94.84}\\
    %\hline
    \specialrule{.1em}{.1em}{.1em}
    \end{tabular}
    }
    \vspace{1mm}
    \caption{Iterations of Recursive inference}
    \label{table:rec_infer}

\end{minipage}
\hfill
\begin{minipage}[b]{0.54\linewidth}
    \scalebox{0.88}{
    \begin{tabular}{c|c|cc}
    \specialrule{.1em}{.1em}{.1em}
    Training Set & \multicolumn{1}{c}{Depth Metrics} & \multicolumn{2}{|c}{Intersection Conf. Metrics} \\
    & CD $\downarrow$  & Rec. (\%) $\uparrow$ & F-score (\%) $\uparrow$  \\ \specialrule{.1em}{.1em}{.1em}
     Mesh          & 0.302  & 96.29 & 94.65 \\ 
     Depth Images  & 1.621  & 92.87 & 88.60\\
    % Point Cloud   &  &  &  &  &  &  &  \\
    \specialrule{.1em}{.1em}{.1em}
    \end{tabular}
    }
    \vspace{1mm}
    \caption{NeuralODF with various fidelity}
    \label{table:var_set}

\end{minipage}
\vspace{-7mm}
\end{table}

==> tables/baselines.tex <==

% \setlength{\tabcolsep}{4pt}
% \begin{table}[h!]
% % \resizebox{0.8\columnwidth}{!}
% {
% %\centering
% \begin{minipage}[b]{0.45\linewidth}\centering
    
% %\scalebox{0.9}{
% \begin{tabular}{l|c|cc}
% \specialrule{.1em}{.1em}{.1em}
% Method & Category & \multicolumn{2}{c}{Depth Metrics} \\
% & & CD $\downarrow$  & F-score (\%) $\uparrow$ \\
% \specialrule{.1em}{.1em}{.1em}
% UDF & Chair & 1.457  & 12.21 \\
% NeuralODF (Ours) & Chair & \textbf{1.105}  & \textbf{13.05} \\
% \specialrule{.1em}{.1em}{.1em}
% \end{tabular}
% %    }
%     \vspace{1mm}
% \caption{Generalization performance of NeuralODF and UDF with the same architecture.
% % \srinath{Add ``Ours'' to NeuralODF --> NeuralODF (Ours). Make best performance \textbf{bold}. Please do that for the table on the right as well. Add citation for UDF.}
% }
% \label{table:gen_base}

% \end{minipage}
% \hfill
% \begin{minipage}[b]{0.45\linewidth}
%  %   \scalebox{0.9}{
% \begin{tabular}{l|c|cc}
% \specialrule{.1em}{.1em}{.1em}
% Method & Category & \multicolumn{2}{c}{Depth Metrics} \\
% & & CD $\downarrow$  & F-score (\%) $\uparrow$ \\
% \specialrule{.1em}{.1em}{.1em}
% NeuralUDF & Car & 1.832  & 2.92 \\
% NeuralODF (Ours) & Car & \textbf{1.904}  & \textbf{2.18} \\
% \specialrule{.1em}{.1em}{.1em}
% \end{tabular}
% %    }
%     \vspace{1mm}
% \caption{Generalization performance of NeuralODF and NeuralUDF}
% \label{table:gen_base2}

% \end{minipage}
% %\vspace{-7mm}
% }
% \end{table}


% \begin{wrapfigure}[20]{r}{0.35\textwidth}
% \vspace{-0.15in}
\begin{table}[h!]
\centering
\scalebox{1}{
    \begin{tabular}{l|c|cc}
        \specialrule{.1em}{.1em}{.1em}
        Category & Method & \multicolumn{2}{c}{CD$\downarrow$} \\
        & & Open & Close \\
        \specialrule{.1em}{.1em}{.1em}
         & NDF~\cite{chibane2020neural} & \textbf{0.059} & - \\
        \multirow{-2}{*}{Airplane} & NeuralODF (Ours) & 0.849 & 0.822 \\
        \hline       
        & IF-Net~\cite{chibane20ifnet} & - & \textbf{0.117} \\
        & NDF~\cite{chibane2020neural} & 0.166 & - \\
        & GIFS~\cite{ye2022gifs} & \textbf{0.127} & - \\
        \multirow{-2}{*}{Car} & NeuralODF (Ours) & 1.089 & 0.862 \\
        \hline
        & IF-Net~\cite{chibane20ifnet} & - & \textbf{0.131} \\
        & NDF~\cite{chibane2020neural} & 0.079 & - \\
        & GIFS~\cite{ye2022gifs} & \textbf{0.074} & - \\
        \multirow{-2}{*}{Chair} & NeuralODF (Ours) & 1.027 & 0.933 \\
        \specialrule{.1em}{.1em}{.1em}
    \end{tabular}
    }
  \vspace{3mm}
  \caption{Point cloud reconstruction comparison on Shapenet dataset.
  \todo{What can we conclude from these results? Our method is}
  }
  \label{table101}
\end{table}

==> tables/nodf_results.tex <==
% \begin{table}
% %\centering
% \begin{minipage}[b]{0.45\linewidth}\centering
    
%     \scalebox{0.5}{
%     \begin{tabular}{lccccc}
%     %\hline
%     \specialrule{.1em}{.1em}{.1em}
%     Method & \multicolumn{2}{c}{Depth Metrics} & \multicolumn{3}{c}{Intersection Conf. Metrics} \\
%     & CD $\downarrow$  & F-score (\%) $\uparrow$ & Rec. (\%) $\uparrow$ & Prec.  (\%) $\uparrow$  & F-score (\%) $\uparrow$  \\ %\hline
%     \specialrule{.1em}{.1em}{.1em}
%     NODF & 0.302  & 24.91 & 96.29 & 93.07  & 94.65\\
%     UDF  & 0.857 & 15.80 & 86.94 & 75.42 & 80.77 \\ 
%     %\hline
%     \specialrule{.1em}{.1em}{.1em}
%     \end{tabular}
%     }
%     \caption{Overfitting performance}
%     \label{table:rec_infer}

% \end{minipage}
%     %\hfill
% \begin{minipage}[b]{0.45\linewidth}

%     \scalebox{0.5}{
%     \begin{tabular}{lccccc}
%     \specialrule{.1em}{.1em}{.1em}
%     Category & \multicolumn{2}{c}{Depth Metrics} & \multicolumn{3}{c}{Intersection Conf. Metrics} \\
%     & CD $\downarrow$  & F-score (\%) $\uparrow$  & Rec. (\%) $\uparrow$ & Prec. (\%) $\uparrow$ & F-score (\%) $\uparrow$   \\
%     \specialrule{.1em}{.1em}{.1em}
%     Airplane & 0.976  & 13.82  & 96.82 & 78.39 & 86.47\\
%     Car & 1.339  & 12.86 & 97.69 & 91.63 & 94.52 \\ 
%     Chair & 1.105  & 13.05  & 96.07 & 85.06 & 90.11\\
%     \specialrule{.1em}{.1em}{.1em}
%     \end{tabular}
%     }
%     \caption{Generalization performance}
%     \label{table:gen}

% \end{minipage}
% \end{table}

\setlength{\tabcolsep}{4pt}
\begin{table}
%\centering
\begin{minipage}[b]{0.45\linewidth}\centering
    
    \scalebox{0.8}{
    \begin{tabular}{l|cc|cc}
    %\hline
    \specialrule{.1em}{.1em}{.1em}
    Method & \multicolumn{2}{c|}{Depth Metrics} & \multicolumn{2}{c}{Intersection Conf. Metrics} \\
    & CD$\downarrow$  & F-score (\%) $\uparrow$ & Rec.(\%) & F-score (\%)  \\ %\hline
    \specialrule{.1em}{.1em}{.1em}
    NeuralODF & 0.302  & 24.91 & 96.29  & 94.65\\
    UDF  & 0.857 & 15.80 & 86.94 & 80.77 \\ 
    %\hline
    \specialrule{.1em}{.1em}{.1em}
    \end{tabular}
    }
    \vspace{1mm}
    \caption{Avg. results on single-object fitting}
    \label{table:sig_infer}

\end{minipage}
\hfill
\begin{minipage}[b]{0.45\linewidth}
    \scalebox{0.7}{
    \begin{tabular}{l|cc|cc}
    \specialrule{.1em}{.1em}{.1em}
    Category & \multicolumn{2}{c|}{Depth Metrics} & \multicolumn{2}{c}{Intersection Conf.} \\
    & CD $\downarrow$  & F-score (\%) $\uparrow$  & Rec. (\%) $\uparrow$ & F-score (\%) $\uparrow$   \\
    \specialrule{.1em}{.1em}{.1em}
    Airplane & 0.976  & 13.82  & 96.82 & 86.47\\
    Car & 1.339  & 12.86 & 97.69 & 94.52 \\ 
    Chair & 1.105  & 13.05  & 96.07 & 90.11\\
    \specialrule{.1em}{.1em}{.1em}
    \end{tabular}
    }
    \vspace{1mm}
    \caption{Generalization of ODF on Shapenet}
    \label{table:gen}

\end{minipage}
\vspace{-7mm}
\end{table}

==> tables/time.tex <==
\setlength{\tabcolsep}{4pt}
\begin{table}
\centering
\scalebox{0.95}{
\begin{tabular}{c|cccc}
\specialrule{.1em}{.1em}{.1em}
ODF & Point Cloud & Depth Map & Mesh & Voxel \\ 
\specialrule{.1em}{.1em}{.1em}
Time Com. & $\mathbb{O}(n)$ & $\mathbb{O}(hw)$ & $\mathbb{O}(n^2)$ & $\mathbb{O}(n^3)$ \\
\specialrule{.1em}{.1em}{.1em}
\end{tabular}
}
\caption{Time complexity of ODF forward mappings. }
\label{table:time}
\end{table}
